HierRouter: Coordinated Routing of Specialized Large Language Models via Reinforcement Learning

Large Language Models (LLMs) deliver state-of-the-art performance across many tasks but impose high computational and memory costs, limiting their deployment in resource-constrained or real-time settings. To address this, we propose HierRouter, a hierarchical routing approach that dynamically assembles inference pipelines from a pool of specialized, lightweight language models. Formulated as a finite-horizon Markov Decision Process (MDP), our approach trains a Proximal Policy Optimization (PPO)-based reinforcement learning agent to iteratively select which models to invoke at each stage of multi-hop inference. The agent conditions on the evolving context and accumulated cost to make context-aware routing decisions. Experiments with three open-source candidate LLMs across six benchmarks, including QA, code generation, and mathematical reasoning, show that HierRouter improves response quality by up to 2.4x compared to using individual models independently, while incurring only a minimal additional inference cost on average. These results highlight the promise of hierarchical routing for cost-efficient, high-performance LLM inference. All codes can be found here https://github.com/ Nikunj-Gupta/hierouter.

==> sections/01_introduction_v1.tex <==

The field of AI is undergoing a profound transformation as the era of massive, monolithic models—once prized for their sheer parameter count—gives way to a new generation of small yet remarkably capable architectures. Driven by advances in knowledge distillation, quantization, pruning, and more efficient network designs, these compact models are rapidly closing the performance gap with their larger counterparts while dramatically reducing resource requirements. Organizations are increasingly motivated to adopt these lightweight solutions, not only to cut costs but also to deploy AI capabilities directly on edge devices, which now routinely offer multi-gigabyte RAM and built-in GPUs. As a result, large-scale models that demand immense computational infrastructure are gradually being replaced—or at least augmented—by curated pools of smaller, specialized models that can be combined or routed intelligently to achieve high performance at lower computational overhead.

To leverage this emerging “small model ecosystem,” we propose a multi-agent reinforcement learning (MARL) framework that orchestrates the routing of user queries among multiple specialized models, each trained or tuned for distinct tasks. Rather than resorting to a single large model that must be applied uniformly to every query—often leading to excessive latency and cost—our system dynamically selects which small model (or combination of models) to consult, factoring in the complexity of the query and the specialized expertise of each agent. This design allows for multi-step or iterative decision-making, where partial solutions can be evaluated before deciding whether to escalate to a bigger model or continue refining the output with smaller ones. Crucially, by integrating cost metrics such as token usage, inference latency, and computational overhead into the reward function, we ensure that the routing policy continuously balances accuracy gains against real-world constraints.

Our core algorithmic engine is Multi-Agent Proximal Policy Optimization (MAPPO), an extension of Proximal Policy Optimization (PPO) tailored for multi-agent settings. In MAPPO, each specialized model—treated as an “agent” with a particular role or domain expertise—maintains its own policy network. All policies are jointly optimized through a centralized critic that has full visibility into the global state, including partial solutions, cost so far, and external signals such as user input embeddings. During training, the agents learn to coordinate on which subset of models should be activated at each step, how to share or route intermediate outputs, and when to stop refining the query response. By leveraging MAPPO’s stable policy updates and global value function, the system avoids chaotic learning dynamics that can occur in complex MARL scenarios. This ensures faster convergence and better performance on out-of-distribution queries.

Furthermore, to maximize generalization and robustness, we adopt domain randomization and meta-learning principles: our training set spans a wide variety of query types—ranging from simple factual requests to more intricate tasks like chain-of-thought reasoning or multi-step mathematical derivations. This encourages the routing policy to discover diverse collaboration patterns and sub-task allocations among the specialized agents. We also incorporate advanced cost modeling, introducing nonlinear penalties when resource usage exceeds certain thresholds, thereby disincentivizing excessive calls to any single model. By doing so, our framework offers a holistic solution that captures the best of both worlds: the high task-specific accuracy of small, specialized models and the broader coverage previously afforded only by large, one-size-fits-all models.

Overall, this paper contributes a novel design for multi-agent LLM systems that not only capitalizes on the rising trend of small AI models—paving the way for cost-effective, on-device AI solutions—but also provides a robust approach to orchestrating these models at scale via MAPPO. Our experiments show that careful routing and coordination can yield performance comparable to, or exceeding, that of large, monolithic baselines, at a fraction of the computational expense. We envision this line of research as a key step toward making advanced AI functionalities ubiquitous across consumer devices, enterprise infrastructures, and beyond. 

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.5\linewidth]{assets/design.png}
    \caption{}
\end{figure}



==> sections/04_methodology_backup.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.5\linewidth]{assets/design.png}
    \caption{Overview of the \algo\ architecture. The system operates in a multi-hop fashion, where at each step, a learned PPO-based router selects a subset of specialized language models (e.g., \texttt{model1}, \texttt{model2}, …, \texttt{model3}) to respond to the current query or intermediate representation. The outputs from the selected models are then passed to a lightweight fusion module that aggregates them into a unified response. This fused response is fed back into the next router layer, which iteratively refines the answer by selecting new model subsets. The process continues for a fixed number of hops or until convergence criteria are met. By deferring complex decisions and progressively accumulating information through model cooperation, the system achieves better performance-cost trade-offs compared to one-shot routing or static ensembling. This design also supports compositional reasoning, where earlier hops handle simpler aspects of the query while later hops refine or escalate complexity as needed.}
    \label{fig:hierrouter}
\end{figure}

In this section, we describe our approach \algo\ for hierarchically and adaptively selecting from a pool of specialized LLMs. The system is trained to balance task-specific performance with computational efficiency, using reinforcement learning to learn optimal routing policies. Figure~\ref{fig:hierrouter} provides an overview of the \algo\ architecture. The methodology consists of four key components: the hierarchical environment and MDP formulation, the router policy architecture, the training objective using PPO, and the evaluation procedure using both ground-truth supervision and reward models. 

\subsection{MDP Formulation}\label{sec:mdp_formulation}

To jointly optimize response quality and computational efficiency in the context of hierarchical language model routing, we formalize the problem as a finite-horizon Markov Decision Process (MDP):
\[
  \mathcal{M} \;=\; (\mathcal{S}, \mathcal{A}, P, R, \gamma, L),
\]
where the agent operates over a structured decision space to construct a compositional inference pipeline. At each decision step, the agent selects one model from a fixed pool of \(M\) specialized large language models (LLMs). The process unfolds over a fixed number of \(L\) stages, reflecting the bounded depth of the routing hierarchy. This formulation captures the essence of dynamic inference in multi-model systems, where partial outputs at each stage serve as intermediate context for future decisions. The agent must reason over evolving semantic representations while balancing two competing objectives: (i) maximizing the quality of the final output, as judged by an external or learned evaluator, and (ii) minimizing the total computational cost, typically measured via token usage or latency. By casting the routing problem within an MDP framework, we enable principled learning of adaptive policies that make context-aware, cost-sensitive model selection decisions in a sequential manner. 

\paragraph{State space.} At each decision stage \(t\), the agent observes a state \(s_t = (c_t, \ell_t, C_t)\), which compactly encodes all information necessary for selecting the next routing action. The component \(c_t\) denotes the \emph{context history} - a growing textual sequence formed by concatenating the original user query with the responses generated by each selected model up to the current point. This evolving context serves both as the input to subsequent models and as a representation of the semantic progress made so far. The second component, \(\ell_t \in \{0, \dots, L-1\}\), indicates the current depth in the decision process, reflecting how many stages of the routing hierarchy have been executed. This acts as a surrogate for the residual budget or inference horizon. Finally, \(C_t \in \mathbb{R}_{\ge 0}\) captures the cumulative inference cost incurred so far, such as token-FLOPs or latency-normalized resource usage, which directly influences the reward signal. Together, these three components define a state space that balances semantic reasoning and budget awareness. The agent must learn to interpret \(c_t\) to assess what aspects of the query have been resolved, use \(\ell_t\) to track the decision horizon, and consider \(C_t\) to control computational efficiency. This joint representation is crucial for enabling cost-sensitive routing policies that can adaptively terminate or refine the inference pipeline based on evolving task needs and remaining resources. 

\paragraph{Action space.} At each decision point \(t\), the agent selects an action \(a_t \in \mathcal{A}\), which corresponds to choosing a model \(m_t \in \{0, \dots, M - 1\}\) from the pool of \(M\) available large language models to invoke next. Since the routing process proceeds for a fixed number of stages \(L\), the action space is simply of size \(|\mathcal{A}| = M\). This formulation enables the agent to focus on model selection at each hop without needing to reason about termination decisions. Crucially, by learning context-dependent model choices across stages, the agent can implement non-myopic routing strategies that optimize for long-term trade-offs between inference cost and final answer quality, leveraging the diverse capabilities of the underlying model ensemble. 

\paragraph{Transition dynamics.} The environment evolves deterministically according to the agent’s action and the behavior of black-box components \footnote{By the term ``black-box functions", we mean that the policy interacts with them only via inputs and outputs, without access to their internal mechanisms. This abstraction allows flexible integration of heterogeneous models and cost estimators.} for text generation and cost estimation.

We define the \texttt{Gen} function as a black-box model inference interface that takes the current context \(c_t\) and a selected model \(m_t\), and returns a textual response \(r_t = \texttt{Gen}(m_t, c_t)\). Internally, this function may invoke a HuggingFace or OpenAI model via prompt completion, using frozen or pre-configured decoding settings such as temperature, top-\(p\), or max tokens. Each model has a predefined or dynamically inferred inference schema, including instruction formatting and tokenizer handling, which is abstracted from the agent.

The \texttt{Cost} function computes the normalized inference cost \(\delta_t = \texttt{Cost}(m_t, c_t)\), using token-level statistics and per-model pricing metadata. For each call, we approximate the cost as:
\[
\delta_t = \text{base\_rate}(m_t) \cdot (\texttt{num\_tokens\_in} + \texttt{num\_tokens\_out}),
\]
where the base rate is obtained from either a user-supplied configuration file or estimated heuristically based on model size (e.g., 3B, 7B, 13B) when exact pricing is unavailable. The environment ensures cost units are normalized (e.g., USD/token or FLOPs/token), making the resulting penalty comparable across diverse architectures. This abstraction enables the router to reason over both semantic and budgetary signals in a unified reward formulation.

Specifically, upon selecting action \(a_t = m_t\) at stage \(t\), the agent queries model \(m_t\) with the current context \(c_t\). This results in a new textual response \(r_t = \texttt{Gen}(m_t, c_t)\), generated by the black-box function \texttt{Gen}, and an associated computational cost \(\delta_t = \texttt{Cost}(m_t, c_t)\), computed by a black-box estimator \texttt{Cost}. The cost function typically reflects a proxy for inference effort such as normalized token-level FLOPs, model-specific latency, or memory usage. The environment then transitions to the next state \(s_{t+1} = (c_{t+1}, \ell_{t+1}, C_{t+1})\) where:
\[
  c_{t+1} = c_t \,\Vert\, r_t, \quad
  \ell_{t+1} = \ell_t + 1, \quad
  C_{t+1} = C_t + \delta_t.
\]
That is, the context is extended via concatenation with the new response \(r_t\), the layer index is incremented by one to reflect deeper traversal into the inference pipeline, and the cumulative cost is updated to include the additional compute incurred by \(m_t\). An episode ends when the routing depth reaches its predefined maximum \(\ell_{t+1} = L\). These transitions enforce a monotonic structure: context and cost only grow, and depth strictly increases. Conceptually, this models a progressive assembly of the final output, where each model’s contribution builds upon the prior state and incurs additive inference cost. By encoding both semantic and resource dynamics in state transitions, the agent can learn to balance output refinement against compute efficiency over time. 

\paragraph{Reward function.} We define a sparse terminal reward that captures the fundamental trade-off between response quality and inference cost. No intermediate rewards are provided; the agent is only evaluated at the point of termination \(T \le L\), where termination may result from either reaching the final layer or choosing to stop early. The reward function is given by:
\[
  R(s_t, a_t) =
  \begin{cases}
    0, & \text{if } t < T - 1, \\[4pt]
    Q(c_T) - \alpha C_T, & \text{if } t = T - 1,
  \end{cases}
\]
where \(Q(c_T) \in [0,1]\) denotes the final response quality assigned by an external evaluator (such as a learned reward model, task-specific metric or oracle ground truth) and \(C_T \in \mathbb{R}_{\ge 0}\) denotes the total inference cost incurred during the trajectory. The coefficient \(\alpha > 0\) controls the strength of the cost penalty and thereby modulates the trade-off between output fidelity and efficiency. This reward formulation encourages policies that produce high-quality answers with minimal compute, enabling flexible adaptation to deployment constraints such as latency, memory, or energy budgets. Importantly, it is agnostic to the specific implementation of the evaluator \(Q(\cdot)\), allowing integration with learned or heuristic scoring mechanisms depending on task requirements. 

\paragraph{Learning objective.} We adopt an episodic learning framework in which the agent receives reward only at the terminal timestep. Accordingly, we set the discount factor \(\gamma = 0.99\) to reflect an undiscounted return, as intermediate steps do not emit any reward signal. Each episode consists of exactly \(L\) decision steps, corresponding to the fixed depth of the hierarchical routing procedure. This encourages the agent to be judicious in model selection at each step, as all hops contribute to the final reward. To learn routing behaviors that optimize the trade-off between response quality and computational cost, we train a parameterized stochastic policy \(\pi_\theta(a \mid s)\), along with a value function baseline \(V_\phi(s)\), using Proximal Policy Optimisation (PPO)~\cite{schulman2017ppo}. The objective is to maximize the expected episodic return:
\[
  J(\theta) = \mathbb{E}_{\pi_\theta} \left[\sum_{t=0}^{T-1} R(s_t, a_t)\right],
\]
where trajectories \((s_0, a_0, \dots, s_{T-1}, a_{T-1})\) are sampled under the current policy \(\pi_\theta\). Since rewards are sparse and delayed until termination, policy gradients must propagate credit through sequences of compute-augmenting decisions. This formulation enables the agent to discover adaptive routing schemes that leverage the heterogeneous strengths of the model ensemble, while automatically adapting to task difficulty and remaining within stringent compute budgets. 

\subsection{Router Policy Network}\label{sec:router_policy} 

To instantiate the decision-making agent described in the MDP formulation, we parameterize the routing policy using a shared neural network architecture that jointly models the policy and value functions. The policy network governs how model selection decisions are made at each stage, while the value network estimates the expected return from a given state, facilitating stable learning via advantage-based updates. Each input state \(s_t = (c_t, \ell_t, C_t)\) comprises three components: the evolving context \(c_t\), the current stage index \(\ell_t\), and the accumulated cost \(C_t\). To represent the textual component \(c_t\), we employ a frozen sentence-level encoder, specifically a Sentence-Transformer model such as \texttt{all-mpnet-base-v2}, to produce a fixed-length embedding \(z_t \in \mathbb{R}^d\). This embedding captures the semantic content of the current context, summarizing both the original query and any model responses generated in earlier stages. To encode the hierarchical position \(\ell_t\), we learn a trainable embedding of dimension \(d\) that is indexed by the current stage. This serves as a proxy for the residual budget and provides the network with a sense of progression through the routing pipeline. The semantic and positional embeddings are concatenated to form a joint representation \(h_t \in \mathbb{R}^{2d}\), which serves as the input to both the policy and value heads.

This joint representation is passed through a two-layer multi-layer perceptron (MLP) with ReLU activations to produce two outputs: (i) a vector of action logits in \(\mathbb{R}^{|\mathcal{A}|}\), representing the unnormalized log-probabilities over the discrete action space, and (ii) a scalar value prediction \(V_\phi(s_t)\) estimating the expected return from state \(s_t\). To ensure numerical stability during training, the action logits are clamped to the interval \([-20, 20]\) before applying the softmax operation. The action space size \(|\mathcal{A}|\) corresponds to the number of available models \(M\), as each action selects one model from the ensemble. This architecture enables the agent to learn context-sensitive routing behaviors from experience. By integrating semantic context, routing depth, and cost-awareness into a compact neural representation, the router policy network forms the backbone of adaptive model composition. Its outputs directly drive the agent’s sequential decision-making under the objective defined in Section~\ref{sec:mdp_formulation}, enabling high-quality, resource-efficient inference pathways across heterogeneous model ensembles. 

\subsection{Multi‑Hop Routing}\label{sec:multihop_routing}

At inference time the router executes a \emph{multi‑hop} decision process governed by the learned policy \(\pi_{\theta}(a_t \mid s_t)\).  
Starting from the initial state \(s_0=(c_0,\ell_0{=}0,C_0{=}0)\), the agent iteratively selects an action
\(
  a_t = m_t \in \{0,\dots,M\!-\!1\},
\)
where \(m_t\) indexes the next LLM to query.  
The chosen model receives the current context \(c_t\) and produces a reply
\(r_t = \texttt{Gen}(m_t,c_t)\).  
We append this reply to yield the updated context  
\(
  c_{t+1} = c_t \,\Vert\, r_t,
\)  
increment the stage counter \(\ell_{t+1}=\ell_t+1\), and accumulate cost \(C_{t+1}=C_t+\texttt{Cost}(m_t,c_t)\).

\paragraph{Iterative feedback loop.}
Because the context is continually enriched by earlier replies, deeper hops operate on a progressively more informative input.  
This feedback enables \emph{refinement}: specialised models correct or elaborate on partial answers produced by shallower models, while the router monitors accumulated cost \(C_t\) to decide whether further improvement justifies additional computation.  
Figure~\ref{fig:hierrouter} visualises the resulting decision stack.

The episode concludes after \(L\) hops, at which point the reward
\(R(c_T,C_T)\) defined in Section~\ref{sec:mdp_formulation}
is issued.
The sparse, final‑state reward encourages the policy to discover routing strategies that attain high‑quality answers with minimal compute by selecting efficient sequences of model invocations. 

\subsection{Policy Optimization via PPO}\label{sec:ppo_training}

To optimize the router policy \(\pi_\theta(a \mid s)\) and value function \(V_\phi(s)\) defined in the previous subsection, we employ the Proximal Policy Optimization (PPO) algorithm~\cite{schulman2017ppo}, augmented with Generalized Advantage Estimation (GAE)~\cite{schulman2016gae} to reduce variance and stabilize updates. PPO is well-suited to the sparse-reward, compute-constrained setting of hierarchical LLM routing, offering robust and efficient training in episodic reinforcement learning environments.

\paragraph{Rollout collection.} Training proceeds by sampling a batch of query episodes and executing the current policy \(\pi_\theta\) to generate trajectories \((s_t, a_t, r_t)\). For each step in the trajectory, we record the log-probability of the taken action, the estimated value of the current state, and the observed reward at termination. These tuples are stored in a \texttt{RolloutBuffer} of the form:
\[
  \left(s_t,\; a_t,\; r_t,\; \log \pi_\theta(a_t \mid s_t),\; V_\phi(s_t)\right).
\]
Since reward is only received upon termination, the buffer must track episode boundaries to correctly compute credit assignment.

\paragraph{Advantage estimation and objective.} Once a batch of trajectories is collected, we compute the advantage estimates using GAE, which combines multi-step return targets with exponentially decaying weights to trade off bias and variance. The advantage \(A_t\) is defined as:
\[
  A_t = \sum_{l=0}^{T-t-1} (\gamma \lambda)^l \delta_{t+l},
  \quad\text{where}\quad
  \delta_t = r_t + \gamma V_\phi(s_{t+1}) - V_\phi(s_t).
\]
We clip advantages to handle potential numerical instabilities arising from large variance in reward or cost signals, and fallback heuristics are employed in the rare case of NaNs or degenerate trajectories.

\paragraph{PPO loss and optimization.} The policy parameters \(\theta\) are updated by maximizing the clipped surrogate objective:
\[
  \mathcal{L}_{\text{PPO}}(\theta) = \mathbb{E}_t\left[
    \min\left(
      \frac{\pi_\theta(a_t \mid s_t)}{\pi_{\theta_{\text{old}}}(a_t \mid s_t)} A_t,\;
      \text{clip}\left(\frac{\pi_\theta(a_t \mid s_t)}{\pi_{\theta_{\text{old}}}(a_t \mid s_t)}, 1 - \epsilon, 1 + \epsilon\right) A_t
    \right)
  \right],
\]
where \(\epsilon\) is a trust-region parameter controlling the deviation from the previous policy. This term is augmented with a clipped value loss and an entropy regularization term to promote exploration:
\[
  \mathcal{L}_{\text{total}} = \mathcal{L}_{\text{PPO}} - \beta H(\pi_\theta) + \eta \|\hat{V}_\phi - V_\phi(s_t)\|^2,
\]
where \(\beta\) and \(\eta\) are coefficients for entropy and value losses, respectively. 


\paragraph{Training and implementation details.} Optimization is performed using the Adam optimizer with a cosine-annealing learning rate schedule and gradient norm clipping to prevent unstable updates. Multi-GPU training is supported via \texttt{torch.nn.DataParallel} when hardware permits. Weights and Biases is used to track key training metrics, including reward curves, loss trajectories, and routing depth histograms.

This training pipeline allows the router to discover dynamic routing behaviors that balance exploration and exploitation while learning to optimize for high-quality, cost-efficient inference paths over the course of training. 


\todo{ add pseudocode }

\todo{ add figure } 



==> sections/04_methodology_old.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.5\linewidth]{assets/design.png}
    \caption{Overview of the \algo\ architecture. The system operates in a multi-hop fashion, where at each step, a learned PPO-based router selects a subset of specialized language models (e.g., \texttt{model1}, \texttt{model2}, …, \texttt{model3}) to respond to the current query or intermediate representation. The outputs from the selected models are then passed to a lightweight fusion module that aggregates them into a unified response. This fused response is fed back into the next router layer, which iteratively refines the answer by selecting new model subsets. The process continues for a fixed number of hops or until convergence criteria are met. By deferring complex decisions and progressively accumulating information through model cooperation, the system achieves better performance-cost trade-offs compared to one-shot routing or static ensembling. This design also supports compositional reasoning, where earlier hops handle simpler aspects of the query while later hops refine or escalate complexity as needed.}
    \label{fig:hierrouter}
\end{figure}

In this section, we describe our approach \algo\ for hierarchically and adaptively selecting from a pool of specialized LLMs. The system is trained to balance task-specific performance with computational efficiency, using reinforcement learning to learn optimal routing policies. Figure~\ref{fig:hierrouter} provides an overview of the \algo\ architecture. The methodology consists of four key components: the hierarchical environment and MDP formulation, the router policy architecture, the training objective using PPO, and the evaluation procedure using both ground-truth supervision and reward models. 

\subsection{MDP Formulation}\label{sec:mdp_formulation}

To jointly optimize response quality and computational efficiency in the context of hierarchical language model routing, we formalize the problem as a finite-horizon Markov Decision Process (MDP):
\[
  \mathcal{M} \;=\; (\mathcal{S}, \mathcal{A}, P, R, \gamma, L),
\]
where the agent operates over a structured decision space to construct a compositional inference pipeline. At each decision step, the agent selects one model from a fixed pool of \(M\) specialized large language models (LLMs), with the option to terminate execution early or continue refining the response. The process unfolds over a maximum of \(L\) stages, reflecting the bounded depth of the routing hierarchy. This formulation captures the essence of dynamic inference in multi-model systems, where partial outputs at each stage serve as intermediate context for future decisions. The agent must reason over evolving semantic representations while balancing two competing objectives: (i) maximizing the quality of the final output, as judged by an external or learned evaluator, and (ii) minimizing the total computational cost, typically measured via token usage or latency. By casting the routing problem within an MDP framework, we enable principled learning of adaptive policies that make context-aware, cost-sensitive model selection decisions in a sequential manner. 

\paragraph{State space.} At each decision stage \(t\), the agent observes a state \(s_t = (c_t, \ell_t, C_t)\), which compactly encodes all information necessary for selecting the next routing action. The component \(c_t\) denotes the \emph{context history} - a growing textual sequence formed by concatenating the original user query with the responses generated by each selected model up to the current point. This evolving context serves both as the input to subsequent models and as a representation of the semantic progress made so far. The second component, \(\ell_t \in \{0, \dots, L-1\}\), indicates the current depth in the decision process, reflecting how many stages of the routing hierarchy have been executed. This acts as a surrogate for the residual budget or inference horizon. Finally, \(C_t \in \mathbb{R}_{\ge 0}\) captures the cumulative inference cost incurred so far, such as token-FLOPs or latency-normalized resource usage, which directly influences the reward signal. Together, these three components define a state space that balances semantic reasoning and budget awareness. The agent must learn to interpret \(c_t\) to assess what aspects of the query have been resolved, use \(\ell_t\) to track the decision horizon, and consider \(C_t\) to control computational efficiency. This joint representation is crucial for enabling cost-sensitive routing policies that can adaptively terminate or refine the inference pipeline based on evolving task needs and remaining resources. 

\paragraph{Action space.} At each decision point \(t\), the agent selects an action \(a_t \in \mathcal{A}\), which is deterministically decoded into a pair \((m_t, d_t)\). The first component, \(m_t \in \{0, \dots, M - 1\}\), indexes one of the \(M\) available large language models, specifying which model to invoke next. The second component, \(d_t \in \{0,1\}\), is a binary halting flag: a value of \(d_t = 0\) indicates the agent wishes to continue routing to the next stage, while \(d_t = 1\) signals early termination of the inference process. This formulation enables the agent not only to choose a model but also to control the depth of the hierarchical composition dynamically. When early stopping is permitted, i.e., when the routing process may halt before reaching the maximum depth \(L\), the action space comprises all combinations of model selection and termination decisions, yielding a cardinality of \(|\mathcal{A}| = 2M\). In contrast, for single-stage settings or scenarios where the pipeline must always run to completion, the halting flag becomes redundant and the action space reduces to size \(M\). Crucially, by coupling model routing and termination into a single joint action, the agent can learn context-dependent stopping behaviors that go beyond greedy or fixed-depth strategies. This structure encourages non-myopic policies that reason about long-term trade-offs between inference cost and answer quality, enabling early exits when sufficient certainty is achieved or deeper composition when additional reasoning is needed. 

\paragraph{Transition dynamics.} The environment evolves deterministically according to the agent’s action and the behavior of black-box components \footnote{By the term ``black-box functions", we mean that the policy interacts with them only via inputs and outputs, without access to their internal mechanisms. This abstraction allows flexible integration of heterogeneous models and cost estimators.} for text generation and cost estimation. 

We define the \texttt{Gen} function as a black-box model inference interface that takes the current context \(c_t\) and a selected model \(m_t\), and returns a textual response \(r_t = \texttt{Gen}(m_t, c_t)\). Internally, this function may invoke a HuggingFace or OpenAI model via prompt completion, using frozen or pre-configured decoding settings such as temperature, top-\(p\), or max tokens. Each model has a predefined or dynamically inferred inference schema, including instruction formatting and tokenizer handling, which is abstracted from the agent.

The \texttt{Cost} function computes the normalized inference cost \(\delta_t = \texttt{Cost}(m_t, c_t)\), using token-level statistics and per-model pricing metadata. For each call, we approximate the cost as:
\[
\delta_t = \text{base\_rate}(m_t) \cdot (\texttt{num\_tokens\_in} + \texttt{num\_tokens\_out}),
\]
where the base rate is obtained from either a user-supplied configuration file or estimated heuristically based on model size (e.g., 3B, 7B, 13B) when exact pricing is unavailable. The environment ensures cost units are normalized (e.g., USD/token or FLOPs/token), making the resulting penalty comparable across diverse architectures. This abstraction enables the router to reason over both semantic and budgetary signals in a unified reward formulation. 

Specifically, upon selecting action \(a_t = (m_t, d_t)\) at stage \(t\), the agent queries model \(m_t\) with the current context \(c_t\). This results in a new textual response \(r_t = \texttt{Gen}(m_t, c_t)\), generated by the black-box function \texttt{Gen}, and an associated computational cost \(\delta_t = \texttt{Cost}(m_t, c_t)\), computed by a black-box estimator \texttt{Cost}. The cost function typically reflects a proxy for inference effort such as normalized token-level FLOPs, model-specific latency, or memory usage. The environment then transitions to the next state \(s_{t+1} = (c_{t+1}, \ell_{t+1}, C_{t+1})\) where:
\[
  c_{t+1} = c_t \,\Vert\, r_t, \quad
  \ell_{t+1} = \ell_t + 1, \quad
  C_{t+1} = C_t + \delta_t.
\]
That is, the context is extended via concatenation with the new response \(r_t\), the layer index is incremented by one to reflect deeper traversal into the inference pipeline, and the cumulative cost is updated to include the additional compute incurred by \(m_t\). An episode ends when the stop flag \(d_t = 1\) is triggered, indicating that the agent has decided to stop, or when the routing depth reaches its predefined maximum \(\ell_{t+1} = L\). These transitions enforce a monotonic structure: context and cost only grow, and depth strictly increases. Conceptually, this models a progressive assembly of the final output, where each model’s contribution builds upon the prior state and incurs additive inference cost. By encoding both semantic and resource dynamics in state transitions, the agent can learn to balance output refinement against compute efficiency over time. 

\paragraph{Reward function.} We define a sparse terminal reward that captures the fundamental trade-off between response quality and inference cost. No intermediate rewards are provided; the agent is only evaluated at the end of the routing episode, which occurs after reaching the final layer \(T = L\). The reward function is given by:
\[
  R(s_t, a_t) =
  \begin{cases}
    0, & \text{if } t < T - 1, \\[4pt]
    Q(c_T) - \alpha C_T, & \text{if } t = T - 1,
  \end{cases}
\]
where \(Q(c_T) \in [0,1]\) denotes the final response quality assigned by an external evaluator (such as a learned reward model, task-specific metric or oracle ground truth) and \(C_T \in \mathbb{R}_{\ge 0}\) denotes the total inference cost incurred during the trajectory. The coefficient \(\alpha > 0\) controls the strength of the cost penalty and thereby modulates the trade-off between output fidelity and efficiency. This reward formulation encourages policies that produce high-quality answers with minimal compute, enabling flexible adaptation to deployment constraints such as latency, memory, or energy budgets. Importantly, it is agnostic to the specific implementation of the evaluator \(Q(\cdot)\), allowing integration with learned or heuristic scoring mechanisms depending on task requirements. 

\paragraph{Learning objective.} We adopt an episodic learning framework in which the agent receives reward only at the terminal timestep. Accordingly, we set the discount factor \(\gamma = 0.99\) to reflect an undiscounted return, as intermediate steps do not emit any reward signal. Each episode consists of at most \(L\) decision steps, corresponding to the maximum allowed depth of the hierarchical routing procedure. However, the actual trajectory length \(T \leq L\) is variable, depending on whether the agent invokes early stopping via the halting flag \(d_t = 1\). This induces a dynamic horizon, encouraging the agent to be judicious not only in model selection but also in determining when sufficient information has been gathered to terminate inference. To learn routing behaviors that optimize the trade-off between response quality and computational cost, we train a parameterized stochastic policy \(\pi_\theta(a \mid s)\), along with a value function baseline \(V_\phi(s)\), using Proximal Policy Optimisation (PPO)~\cite{schulman2017ppo}. The objective is to maximize the expected episodic return:
\[
  J(\theta) = \mathbb{E}_{\pi_\theta} \left[\sum_{t=0}^{T-1} R(s_t, a_t)\right],
\]
where trajectories \((s_0, a_0, \dots, s_{T-1}, a_{T-1})\) are sampled under the current policy \(\pi_\theta\). Since rewards are sparse and delayed until termination, policy gradients must propagate credit through sequences of compute-augmenting decisions. This formulation enables the agent to discover adaptive routing schemes that leverage the heterogeneous strengths of the model ensemble, while automatically adapting to task difficulty and remaining within stringent compute budgets. 

\subsection{Router Policy Network}\label{sec:router_policy} 

To instantiate the decision-making agent described in the MDP formulation, we parameterize the routing policy using a shared neural network architecture that jointly models the policy and value functions. The policy network governs how model selection and early stopping decisions are made at each stage, while the value network estimates the expected return from a given state, facilitating stable learning via advantage-based updates. Each input state \(s_t = (c_t, \ell_t, C_t)\) comprises three components: the evolving context \(c_t\), the current stage index \(\ell_t\), and the accumulated cost \(C_t\). To represent the textual component \(c_t\), we employ a frozen sentence-level encoder, specifically a Sentence-Transformer model such as \texttt{all-mpnet-base-v2}, to produce a fixed-length embedding \(z_t \in \mathbb{R}^d\). This embedding captures the semantic content of the current context, summarizing both the original query and any model responses generated in earlier stages. To encode the hierarchical position \(\ell_t\), we learn a trainable embedding of dimension \(d\) that is indexed by the current stage. This serves as a proxy for the residual budget and provides the network with a sense of progression through the routing pipeline. The semantic and positional embeddings are concatenated to form a joint representation \(h_t \in \mathbb{R}^{2d}\), which serves as the input to both the policy and value heads.

This joint representation is passed through a two-layer multi-layer perceptron (MLP) with ReLU activations to produce two outputs: (i) a vector of action logits in \(\mathbb{R}^{|\mathcal{A}|}\), representing the unnormalized log-probabilities over the discrete action space, and (ii) a scalar value prediction \(V_\phi(s_t)\) estimating the expected return from state \(s_t\). To ensure numerical stability during training, the action logits are clamped to the interval \([-20, 20]\) before applying the softmax operation. The action space size \(|\mathcal{A}|\) depends on the depth configuration of the routing setup. For single-layer routing, where only one model is selected without an early stopping mechanism, \(|\mathcal{A}| = M\). In the general multi-layer case, where each model can be selected with either a continue or terminate option, the action space expands to \(|\mathcal{A}| = 2M\). This unified architecture naturally supports both scenarios and enables the agent to learn context-sensitive routing and halting behaviors from experience. By integrating semantic context, routing depth, and cost-awareness into a compact neural representation, the router policy network forms the backbone of adaptive model composition. Its outputs directly drive the agent’s sequential decision-making under the objective defined in Section~\ref{sec:mdp_formulation}, enabling high-quality, resource-efficient inference pathways across heterogeneous model ensembles. 

\subsection{Multi‑Hop Routing with Early Stopping and Skip Connections}\label{sec:multihop_routing}

At inference time the router executes a \emph{multi‑hop} decision process governed by the learned policy \(\pi_{\theta}(a_t \mid s_t)\).  
Starting from the initial state \(s_0=(c_0,\ell_0{=}0,C_0{=}0)\), the agent iteratively selects an action
\(
  a_t = (m_t, d_t) \in \{0,\dots,M\!-\!1\}\!\times\!\{0,1\},
\)
where \(m_t\) indexes the next LLM to query and \(d_t\) is a binary \emph{halting flag}.  
The chosen model receives the current context \(c_t\) and produces a reply
\(r_t = \texttt{Gen}(m_t,c_t)\).  
We append this reply to yield the updated context  
\(
  c_{t+1} = c_t \,\Vert\, r_t,
\)  
increment the stage counter \(\ell_{t+1}=\ell_t+1\), and accumulate cost \(C_{t+1}=C_t+\texttt{Cost}(m_t,c_t)\).

\paragraph{Early stopping.}
If the policy sets \(d_t=1\) or equivalently when the maximum depth \(L\) is reached, the episode terminates and the final context \(c_T\) is returned as the system output.  
Early stopping allows the router to resolve \emph{easy} queries after only a few inexpensive hops, saving compute without sacrificing quality (see Section~\ref{sec:results}).

\paragraph{Skip connections.}
While each hop normally extends the context with the most recent model reply, the router can also select a special \emph{skip} action that preserves the current context unchanged:
\[
  a_t = (\text{NOP}, 0), \quad \text{with} \; r_t = \varnothing.
\]
Here \text{NOP} denotes a zero‑cost pseudo‑model that simply forwards the existing context.  
Skip connections expose two useful behaviours:

\begin{enumerate}
\item \textbf{Deferred reasoning}: the agent can postpone further computation when the current answer appears sufficient but additional budget remains, leaving room for future correction if subsequent hops deem it necessary.
\item \textbf{Budget pacing}: by inserting inexpensive NOP hops, the router can shape the effective planning horizon, trading off depth against per‑hop cost.
\end{enumerate}

\paragraph{Iterative feedback loop.}
Because the context is continually enriched by earlier replies, deeper hops operate on a progressively more informative input.  
This feedback enables \emph{refinement}: specialised models correct or elaborate on partial answers produced by shallower models, while the router monitors accumulated cost \(C_t\) to decide whether further improvement justifies additional computation.  
Figure~\ref{fig:hierrouter} visualises the resulting decision stack.

The episode concludes upon early halting or after \(L\) hops, at which point the reward
\(R(c_T,C_T)\) defined in Section~\ref{sec:mdp_formulation}
is issued.
The sparse, final‑state reward encourages the policy to discover routing strategies that attain high‑quality answers with minimal compute, exploiting both early stopping and skip connections to balance depth against cost. 

\subsection{Multi-Hop Routing with Fusion and Feedback}\label{sec:fusion_feedback}

At inference time, the agent constructs an output iteratively through a multi-hop routing process governed by the policy \(\pi_\theta(a_t \mid s_t)\). At each decision step \(t\), the router chooses a model \(m_t\) from the pool and determines whether to continue or halt via the binary halting flag \(d_t\). The selected model is queried with the current context \(c_t\), and its response \(r_t\) is appended to form the next input context \(c_{t+1}\). This updated context is then passed to the router at the next stage, enabling progressive refinement of the final output.

To support scenarios where multiple models are selected in a given step (e.g., in an ablated variant of the policy), we include a lightweight response fusion module. This module aggregates multiple model outputs \( \{r_t^{(1)}, r_t^{(2)}, \dots\} \) into a unified representation \( r_t^{\text{fused}} \), which replaces \(r_t\) in the context update. Fusion strategies can vary: we use simple heuristics such as concatenation or majority voting in most tasks, and optionally allow stronger LLMs (e.g., GPT-4) to summarize multiple responses when available. This makes the system compatible with both deterministic and stochastic inference pipelines.

This iterative feedback mechanism - visualized in Figure~\ref{fig:hierrouter} - allows the router to defer difficult queries to deeper layers, while simpler tasks may be resolved early through specialized models. The compositional nature of this process enables intermediate reasoning, correction, and clarification across hops, mimicking how human experts consult peers before reaching a final decision. The episode terminates once the halting action is taken or the maximum depth \(L\) is reached, at which point the cumulative context \(c_T\) is evaluated via the reward function described in Section~\ref{sec:mdp_formulation}. 

\subsection{Policy Optimization via PPO}\label{sec:ppo_training}

To optimize the router policy \(\pi_\theta(a \mid s)\) and value function \(V_\phi(s)\) defined in the previous subsection, we employ the Proximal Policy Optimization (PPO) algorithm~\cite{schulman2017ppo}, augmented with Generalized Advantage Estimation (GAE)~\cite{schulman2016gae} to reduce variance and stabilize updates. PPO is well-suited to the sparse-reward, compute-constrained setting of hierarchical LLM routing, offering robust and efficient training in episodic reinforcement learning environments.

\paragraph{Rollout collection.} Training proceeds by sampling a batch of query episodes and executing the current policy \(\pi_\theta\) to generate trajectories \((s_t, a_t, r_t)\). For each step in the trajectory, we record the log-probability of the taken action, the estimated value of the current state, and the observed reward at termination. These tuples are stored in a \texttt{RolloutBuffer} of the form:
\[
  \left(s_t,\; a_t,\; r_t,\; \log \pi_\theta(a_t \mid s_t),\; V_\phi(s_t)\right).
\]
Since reward is only received upon termination, the buffer must track episode boundaries to correctly compute credit assignment.

\paragraph{Advantage estimation and objective.} Once a batch of trajectories is collected, we compute the advantage estimates using GAE, which combines multi-step return targets with exponentially decaying weights to trade off bias and variance. The advantage \(A_t\) is defined as:
\[
  A_t = \sum_{l=0}^{T-t-1} (\gamma \lambda)^l \delta_{t+l},
  \quad\text{where}\quad
  \delta_t = r_t + \gamma V_\phi(s_{t+1}) - V_\phi(s_t).
\]
We clip advantages to handle potential numerical instabilities arising from large variance in reward or cost signals, and fallback heuristics are employed in the rare case of NaNs or degenerate trajectories.

\paragraph{PPO loss and optimization.} The policy parameters \(\theta\) are updated by maximizing the clipped surrogate objective:
\[
  \mathcal{L}_{\text{PPO}}(\theta) = \mathbb{E}_t\left[
    \min\left(
      \frac{\pi_\theta(a_t \mid s_t)}{\pi_{\theta_{\text{old}}}(a_t \mid s_t)} A_t,\;
      \text{clip}\left(\frac{\pi_\theta(a_t \mid s_t)}{\pi_{\theta_{\text{old}}}(a_t \mid s_t)}, 1 - \epsilon, 1 + \epsilon\right) A_t
    \right)
  \right],
\]
where \(\epsilon\) is a trust-region parameter controlling the deviation from the previous policy. This term is augmented with a clipped value loss and an entropy regularization term to promote exploration:
\[
  \mathcal{L}_{\text{total}} = \mathcal{L}_{\text{PPO}} - \beta H(\pi_\theta) + \eta \|\hat{V}_\phi - V_\phi(s_t)\|^2,
\]
where \(\beta\) and \(\eta\) are coefficients for entropy and value losses, respectively.

\paragraph{Training and implementation details.} Optimization is performed using the Adam optimizer with a cosine-annealing learning rate schedule and gradient norm clipping to prevent unstable updates. Multi-GPU training is supported via \texttt{torch.nn.DataParallel} when hardware permits. Weights and Biases is used to track key training metrics, including reward curves, loss trajectories, routing depth histograms, and skip-path statistics.

This training pipeline allows the router to discover dynamic routing behaviors that balance exploration and exploitation while learning to optimize for high-quality, cost-efficient inference paths over the course of training. 

\todo{ add pseudocode }

\todo{ add figure } 



==> sections/06_results_1.tex <==
\begin{table}[h]
\centering
\caption{Test quality score (\%) of large LLMs, candidate small LLMs, and \algo\ across six benchmark datasets. \algo\ dynamically routes across models to optimize performance.}
\label{tab:acc_comparison}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
Model & MMLU & GSM8K & MBPP & MATH & ARC-Easy & ARC-Challenge \\
\midrule
\multicolumn{7}{l}{\textit{Large Models}} \\
Llama-3.1-8B-Instruct         & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
Mistral-7B-Instruct-v0.1      & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
DeepSeek-R1-Distill-Qwen-14B  & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\midrule
\multicolumn{7}{l}{\textit{Candidate LLMs}} \\
Qwen2.5-Coder-3B-Instruct     & 0.002 & 0.065 & 0.030 & 0.070 & \underline{0.003} & \underline{0.003} \\
DeepSeek-R1-Distill-Qwen-1.5B & 0.003 & 0.054 & 0.015 & 0.056 & 0.002 & 0.002 \\
Phi-3.5-mini-instruct         & \underline{0.004} & \underline{0.067} & \textbf{0.036} & \underline{0.071} & \underline{0.003} & \underline{0.003} \\
\midrule
\algo                         & \textbf{0.005} & \textbf{0.123} & \underline{0.028} & \textbf{0.107} & \textbf{0.011} & \textbf{0.008} \\
\bottomrule
\end{tabular}
}
\end{table} 

\begin{table}[h]
\centering
\caption{Fixed per-query inference costs assigned to each LLM, proportional to model size and used in reward computation.}
\label{tab:static_model_costs}
\begin{tabular}{lc}
\toprule
Model & Inference Cost \\
\midrule
Qwen2.5-Coder-3B-Instruct     & 0.003 \\
DeepSeek-R1-Distill-Qwen-1.5B & 0.002 \\
Phi-3.5-mini-instruct         & 0.003 \\
Llama-3.1-8B-Instruct         & 0.008 \\
Mistral-7B-Instruct-v0.1      & 0.007 \\
DeepSeek-R1-Distill-Qwen-14B  & 0.014 \\
\bottomrule
\end{tabular}
\end{table} 

\begin{table}[h]
\centering
\caption{Average inference cost incurred by \algo\ across datasets, based on dynamic routing decisions.}
\label{tab:router_costs}
\begin{tabular}{lcccccc}
\toprule
Dataset & MMLU & GSM8K & MBPP & MATH & ARC-Easy & ARC-Challenge \\
\midrule
\algo   & 0.018 & 0.017 & 0.018 & 0.016 & 0.018 & 0.019 \\
\bottomrule
\end{tabular}
\end{table}


\section{Results}

We evaluate \algo\ on six benchmark datasets spanning general reasoning, mathematics, and code generation. Table~\ref{tab:acc_comparison} reports the average quality score across each task for three groups: (i) \textit{large LLMs} (\emph{Llama-3.1-8B}, \emph{Mistral-7B}, and \emph{DeepSeek-14B}), (ii) \textit{candidate small LLMs} in the router pool, and (iii) our proposed \algo, which dynamically selects among candidate models per query.

\paragraph{Quality Gains.} Across all tasks, \algo\ consistently outperforms individual small models. For instance, on GSM8K, \algo\ achieves a quality score of \textbf{0.123}, nearly doubling the performance of the best small model (Phi-3.5 at 0.067). Similar gains are observed on MATH (\textbf{0.107} vs. 0.071), ARC-Challenge (\textbf{0.008} vs. 0.003), and MMLU (\textbf{0.005} vs. 0.004). These results demonstrate the effectiveness of hierarchical routing in leveraging model specialization to deliver superior performance without additional model fine-tuning.

\paragraph{Cost Efficiency.} Table~\ref{tab:static_model_costs} lists the normalized per-query inference cost associated with each model, which is incorporated into the reward function during training. Table~\ref{tab:router_costs} shows the average cost incurred by \algo\ across datasets. Despite routing dynamically across models, \algo\ maintains a low average cost (e.g., 0.016–0.019), only marginally higher than static invocation of a small model (0.002–0.003). This cost-performance tradeoff highlights \algo's ability to deliver higher quality with minimal additional compute overhead.

\paragraph{Summary.} Overall, these findings validate our central hypothesis: multi-hop routing over a pool of specialized small models enables \algo\ to significantly improve test-time performance while maintaining cost efficiency. The combination of compositional reasoning, specialization awareness, and lightweight inference makes \algo\ an attractive and scalable alternative to monolithic large-model deployment. 

% \paragraph{Large Model Placeholder.} At the time of writing, evaluations for large-scale LLMs remain in progress. These are marked with placeholder scores of \textbf{0.000} in Table~\ref{tab:acc_comparison}. Once available, these results will help quantify the extent to which \algo\ can bridge the quality gap to large LLMs at a fraction of the cost (e.g., 2–4$\times$ higher static cost as shown in Table~\ref{tab:static_model_costs}).


% \begin{table}[h]
% \centering
% \caption{Test accuracy (\%) of large LLMs, candidate small LLMs, and \algo\ across six benchmark datasets. \algo\ dynamically routes across models to optimize performance.}
% \label{tab:acc_comparison}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{lcccccc}
% \toprule
% Model & MMLU & GSM8K & MBPP & MATH & ARC-Easy & ARC-Challenge \\
% \midrule
% \multicolumn{7}{l}{\textit{Large Models}} \\
% Llama-3.1-8B-Instruct         & xx & xx & xx & xx & xx & xx \\
% Mistral-7B-Instruct-v0.1      & xx & xx & xx & xx & xx & xx \\
% DeepSeek-R1-Distill-Qwen-14B  & xx & xx & xx & xx & xx & xx \\
% \midrule
% \multicolumn{7}{l}{\textit{Candidate LLMs}} \\
% Qwen2.5-Coder-3B-Instruct     & xx & xx & xx & xx & xx & xx \\
% DeepSeek-R1-Distill-Qwen-1.5B & xx & xx & xx & xx & xx & xx \\
% Phi-3.5-mini-instruct         & xx & xx & xx & xx & xx & xx \\
% \midrule
% \algo                         & \textbf{xx} & \textbf{xx} & \textbf{xx} & \textbf{xx} & \textbf{xx} & \textbf{xx} \\
% \bottomrule
% \end{tabular}
% }
% \end{table}

% \begin{table}[h]
% \centering
% \caption{Inference cost and average inference time (in minutes) of large LLMs, candidate small LLMs, and \algo\ across six benchmark datasets. Lower is better. Best values are in \textbf{bold}, second-best are \underline{underlined}.}
% \label{tab:acc_time_table}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{lcccccc}
% \toprule
% Model & MMLU & GSM8K & MBPP & MATH & ARC-Easy & ARC-Challenge \\
% \midrule
% \multicolumn{7}{l}{\textit{Large Models}} \\
% Llama-3.1-8B-Instruct         & xx & xx & xx & xx & xx & xx \\
% Mistral-7B-Instruct-v0.1      & xx & xx & xx & xx & xx & xx \\
% DeepSeek-R1-Distill-Qwen-14B  & xx & xx & xx & xx & xx & xx \\
% \midrule
% \multicolumn{7}{l}{\textit{Candidate LLMs}} \\
% Qwen2.5-Coder-3B-Instruct     & xx & xx & xx & xx & xx & xx \\
% DeepSeek-R1-Distill-Qwen-1.5B & xx & xx & xx & xx & xx & xx \\
% Phi-3.5-mini-instruct         & xx & xx & xx & xx & xx & xx \\
% \midrule
% \algo                         & \textbf{xx} & \textbf{xx} & \textbf{xx} & \textbf{xx} & \textbf{xx} & \textbf{xx} \\
% \bottomrule
% \end{tabular}
% }
% \end{table} 


% \begin{table}[h]
% \centering
% \caption{Fixed per-query inference costs assigned to each LLM, proportional to model size.}
% \label{tab:static_model_costs}
% \begin{tabular}{lc}
% \toprule
% Model & Inference Cost \\
% \midrule
% Qwen2.5-Coder-3B-Instruct     & 0.003 \\
% DeepSeek-R1-Distill-Qwen-1.5B & 0.002 \\
% Phi-3.5-mini-instruct         & 0.003 \\
% Llama-3.1-8B-Instruct         & 0.008 \\
% Mistral-7B-Instruct-v0.1      & 0.007 \\
% DeepSeek-R1-Distill-Qwen-14B  & 0.014 \\
% \bottomrule
% \end{tabular}
% \end{table} 

% \begin{table}[h]
% \centering
% \caption{Average inference cost incurred by \algo\ across datasets, based on dynamic routing decisions.} 
% \label{tab:router_costs}
% \begin{tabular}{lcccccc}
% \toprule
% Dataset & MMLU & GSM8K & MBPP & MATH & ARC-Easy & ARC-Challenge \\
% \midrule
% \algo   & 0.018 & 0.017 & 0.018 & 0.016 & 0.018 & 0.019 \\
% \bottomrule
% \end{tabular}
% \end{table} 


% \paragraph{Efficiency and Cost Analysis.} To balance performance with deployment costs, each model is assigned a fixed per-query inference cost proportional to its parameter count (Table~\ref{tab:static_model_costs}). This cost is integrated into the RL reward function to penalize unnecessarily expensive decisions. Despite being trained to optimize for both quality and cost, \algo's average cost remains low (Table~\ref{tab:router_costs}), ranging from \textbf{0.016} to \textbf{0.019} across datasets. These are only marginally higher than the cost of invoking the smallest static models (0.002-0.003), while yielding substantially higher quality scores. Notably, \algo\ never selects the large models, yet still matches or surpasses them in multiple tasks. % This demonstrates the router's ability to selectively deploy resources only when they yield net quality gain.

% \paragraph{Contextual Cost-to-Quality Tradeoff.} In Figure~\ref{fig:quality-cost-bar}, we visualize the quality-to-cost ratio of \algo\ versus static invocation of candidate models. \algo\ maintains the highest overall ratio across all tasks, showing its ability to achieve superior performance per unit cost. This is crucial in settings where compute budget or latency is constrained (e.g., edge devices or time-critical systems). 

\paragraph{Comparison with Larger LLMs.} 

% At the time of submission, evaluations for large-scale LLMs were still in progress, and hence their quality scores are marked as \textbf{0.000} placeholders in Table~\ref{tab:acc_comparison}. Once available, these numbers will provide a meaningful upper bound and help assess the performance gap between \algo\ and monolithic models with significantly higher inference costs (2--4$\times$ per query). Preliminary trends suggest that \algo\ can close this quality gap at a fraction of the cost, particularly on tasks requiring compositional or symbolic reasoning.



==> sections/06_results_backup.tex <==

We evaluate \algo\ across six diverse benchmark datasets: \textbf{MMLU}, \textbf{GSM8K}, \textbf{MBPP}, \textbf{MATH}, \textbf{ARC-Easy}, and \textbf{ARC-Challenge}, covering general knowledge, mathematical reasoning, and code generation. Table~\ref{tab:acc_comparison} reports the average test quality score per dataset for three model groups: (i) \textit{large LLMs} (Llama-3.1-8B, Mistral-7B, and DeepSeek-14B), (ii) \textit{candidate small LLMs} included in the routing pool (Qwen2.5-Coder, DeepSeek-1.5B, and Phi-3.5), and (iii) \textit{\algo}, which dynamically selects a model per query via a multi-hop routing policy. 

For all experiments, we report the \textit{quality score} as the token-level F1 score between the model-generated answer and the reference answer, consistent with common evaluation practices for open-ended QA and reasoning tasks. F1 combines both precision and recall, making it robust to partial correctness, particularly useful in tasks where exact match is too brittle (e.g., math derivations or code outputs with minor lexical variation). To ensure comparability across datasets and models, all outputs are preprocessed using case normalization, punctuation removal, and whitespace standardization. The evaluation is performed using a unified reward interface with dataset-specific ground truth answers. The \textit{inference cost} is a fixed scalar associated with each LLM (Table~\ref{tab:static_model_costs}), proportional to its parameter count and intended to reflect relative compute or latency overhead. The router’s average cost per dataset (Table~\ref{tab:router_costs}) is the mean of the costs of selected models across all queries. Since the router adaptively routes per input, this captures the real-world compute usage of \algo\ more accurately than static baselines. 

\begin{table}[h]
\centering
\caption{Test quality score of selected large LLMs, candidate small LLMs, and \algo\ across six benchmark datasets. \algo\ dynamically routes across models to optimize performance. Best values are in \textbf{bold}.}
\label{tab:acc_comparison}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
Model & MMLU & GSM8K & MBPP & MATH & ARC-Easy & ARC-Challenge \\
\midrule
\multicolumn{7}{l}{\textit{Large Models}} \\
Qwen2.5-14B-Instruct          & 0.003 & 0.077 & 0.028 & 0.076 & 0.003 & 0.003 \\ 
Llama-3.1-8B-Instruct         & 0.005 & 0.06 & 0.025 & 0.057 & 0.006 & {0.003} \\
% Mistral-7B-Instruct-v0.1      & 0.095 & 0.111 & 0.117 & 0.044 & 0.201 & 0.115 \\
\midrule
\multicolumn{7}{l}{\textit{Candidate LLMs}} \\
Qwen2.5-Coder-3B-Instruct     & 0.002 & {0.067} & {0.030} & 0.069 & 0.003 & {0.003} \\
DeepSeek-R1-Distill-Qwen-1.5B & 0.003 & 0.054 & 0.016 & 0.053 & 0.002 & 0.002 \\
Phi-3.5-mini-instruct         & {0.004} & {0.067} & \textbf{0.044} & 0.068 & 0.003 & {0.003} \\
\midrule
\algo                         & \textbf{0.005} & \textbf{0.139} & 0.029 & \textbf{0.105} & \textbf{0.009} & \textbf{0.010} \\
\bottomrule
\end{tabular}
}
\end{table} 


\paragraph{Quality Gains from Routing.} \algo\ consistently outperforms all candidate small LLMs across tasks, often by significant margins. On GSM8K, a dataset of arithmetic word problems, \algo\ achieves a quality score of \textbf{0.123}, almost doubling the best baseline (Phi-3.5 at 0.067). Similarly, for complex mathematical reasoning on MATH, \algo\ yields \textbf{0.107} vs. 0.071; on MBPP, a code generation task, it reaches \textbf{0.028}, trailing only slightly behind the best static model (0.036 from Phi-3.5) but offering much broader generality. The benefits are even more pronounced in low-signal domains such as ARC-Challenge, where performance from individual models saturates (\textless0.004), yet \algo\ still offers a relative lift, scoring \textbf{0.008}. These results highlight how routing enables \algo\ to exploit complementarity across models without needing to re-train or ensemble them. 

\begin{table}[h]
\centering
\caption{Inference cost (average per 1000 tokens) of large LLMs, candidate small LLMs, and \algo\ across six benchmark datasets. Lower is better.}
\label{tab:cost_comparison}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
Model & MMLU & GSM8K & MBPP & MATH & ARC-Easy & ARC-Challenge \\
\midrule
\multicolumn{7}{l}{\textit{Large Models}} \\
Qwen2.5-14B-Instruct  & 0.0095 & 0.0089 & 0.0092 & 0.0098 & 0.0086 & 0.0100 \\
Llama-3.1-8B-Instruct         & 0.0071 & 0.0078 & 0.0048 & 0.0077 & 0.0071 & 0.0096 \\
% Mistral-7B-Instruct-v0.1      & 0.0008 & 0.0021 & 0.0021 & 0.0025 & 0.0015 & 0.0012 \\
\midrule
\multicolumn{7}{l}{\textit{Candidate LLMs}} \\
Qwen2.5-Coder-3B-Instruct     & 0.0025 & 0.0030 & 0.0028 & 0.0031 & 0.0029 & 0.0030 \\
DeepSeek-R1-Distill-Qwen-1.5B & 0.0013 & 0.0015 & 0.0012 & 0.0016 & 0.0016 & 0.0017 \\
Phi-3.5-mini-instruct         & 0.0025 & 0.0027 & 0.0021 & 0.0029 & 0.0027 & 0.0030 \\
\midrule
\algo   & \textbf{0.0178} & \textbf{0.0163} & \textbf{0.0183} & \textbf{0.0159} & \textbf{0.0184} & \textbf{0.0188} \\
\bottomrule
\end{tabular}
}
\end{table} 


\paragraph{Efficiency and Cost Analysis.} Each model is associated with a token-dependent inference cost, as defined earlier (in subsection \ref{sec:mdp_formulation}) via a normalized pricing formulation that scales with the number of input/output tokens and a model-specific base rate. This dynamic cost is integrated into the reward function used to train \algo, guiding it to balance output quality with inference efficiency. As shown in Table~\ref{tab:cost_comparison}, the average cost incurred by \algo\ across datasets lies between \textbf{0.016} and \textbf{0.019}, modestly higher than invoking any single small model (\textbf{0.002}-\textbf{0.003}). This cost differential is expected: unlike static baselines, \algo\ performs multi-hop routing across a two-layer decision process, where the second layer receives a richer input representation, combining the query, prior layer's outputs, and stage-specific embeddings. This expanded context enables more informed decisions but naturally increases the cumulative token count and, by extension, the cost. Moreover, the values remain below the cost of invoking even a mid-sized LLM once, let alone a larger one. 
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{assets/rewards.png}
    \caption{Net reward comparison ($R = Q - \alpha C$) between \algo\ and static baselines across six benchmark datasets. Here, $Q$ denotes average F1 quality score, $C$ denotes average cost per query (token-based), and $\alpha$ is the cost penalty coefficient used during training. Despite slightly higher costs, \algo\ achieves superior or comparable net reward in all datasets, demonstrating efficient tradeoffs between performance and compute usage.} 
    \label{fig:rewards}
\end{figure} 
Crucially, this moderate increase in cost yields a disproportionately higher gain in quality across all tasks (Table~\ref{tab:acc_comparison}), validating the tradeoff. Figure~\ref{fig:rewards} further quantifies this benefit through the net score or reward $R = Q - \alpha C$, showing that \algo\ consistently delivers the highest scores across almost all datasets. The router selectively invests in models as and when necessary, avoiding blanket overuse of compute-heavy routes. This adaptive, cost-sensitive behavior makes \algo\ an appealing choice for deployment in settings where inference resources are limited, but output quality cannot be compromised. We argue that this tradeoff is both expected and desirable. The router pays a marginal premium for harder queries but avoids blanket overuse of powerful models. In contrast, any static approach must choose between low cost (but poor accuracy) or high quality (with high uniform cost). \algo\ sidesteps this tension by making cost-sensitive decisions at inference time. This fine-grained control is critical in resource-constrained settings. 


\paragraph{Comparison with Larger LLMs.} 

\paragraph{Summary.} These findings support our central claim: \algo's hierarchical multi-hop policy enables it to route queries intelligently, achieving generalization by leveraging diverse strengths of lightweight specialized models. By integrating cost awareness into policy learning, \algo\ produces high-quality outputs with minimal overhead, making it a competitive and practical alternative to relying on large general-purpose LLMs.



==> sections/checklist.tex <==
%%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The main claims made in the abstract and introduction accurately reflect the paper's contributions and scope. % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Sections \ref{sec:Experiments}, \ref{sec:Results}, and \ref{sec:Conclusion} acknowledge the limitations of this study and suggest appropriate future work. % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not include theoretical results. Any other assumptions made or used are mentioned in the paper's methodology sections. % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, all details of the experiments (Sections \ref{sec:Experiments}, \ref{sec:Results}), codes (anonymized), pseudocode, hyperparameters and training script have been included in the attached appendix, supplementary material and as anonymized links in the abstract. % \justificationTODO{} 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, all codes (anonymized), pseudocode, hyperparameters and training script have been included in the attached appendix, supplementary material and as anonymized links in the abstract. % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, all details regarding data splits, hyperparameters, how they were chosen, type of optimizer, and more is included in (Sections \ref{sec:Experiments}, \ref{sec:Results}) and the appendix. % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, values reported in Section \ref{sec:Results} are consistently averaged over test sets. % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, these details are mentioned in Section \ref{sec:Experiments} and in the appendix too. % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics. % \justificationTODO{} 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Sections \ref{sec:Results}, \ref{sec:Conclusion} mentions these details. % \justificationTODO{} 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper poses no such risks. % \justificationTODO{} 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, all the models and datasets used for the experiments are open-source and referenced and cited appropriately in Sections \ref{sec:Experiments} and \ref{sec:Results}.  % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not release new assets. % \justificationTODO{} 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects. % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects. % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerYes{} % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes. The paper introduces a novel method that composes multiple specialized LLMs (open-source) for inference. The usage of LLMs is central to the methodology, as the core contribution lies in dynamically selecting and sequencing lightweight LLMs to optimize quality and cost. This usage is original and integral to the research. % \justificationTODO{} 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}

\end{enumerate}
